A Survey on Network Tomography with Network Coding

The overhead of internal network monitoring motivates techniques of network tomography. Network coding (NC) presents a new opportunity for network tomography as NC introduces topology-dependent correlation that can be further exploited in topology estimation. Compared with traditional methods, network tomography with NC has many advantages such as the improvement of tomography accuracy and the reduction of complexity in choosing monitoring paths. In this paper we first introduce the problem of tomography with NC and then propose the taxonomy criteria to classify various methods. We also present existing solutions and future trend. We expect that our comprehensive review on network tomography with NC can serve as a good reference for researchers and practitioners working in the area.

==> RelatedWork.tex <==
\vspace{-0.1cm}
\section{Related work}
\label{sec::related work}
\vspace{-0.1cm}

Y. Vardi was one of the first to rigorously study the problem of inferring routing topology and coined the term network tomography~\cite{Y.Var::NTESD::1996} due to the similarity between network inference and medical tomography. According to the type of data acquisition and the performance parameters of interest~\cite{RuiCastro::NTRecDeve::2004}, network tomography can be classified into (1) link-level parameter estimation based on end-to-end, path-level traffic measurements and (2) sender-receiver path-level traffic intensity estimation based on link-level traffic measurements. According to the purpose of network tomography, network tomography can also be categorized into topology discovery, link loss rates estimation, and delay tomography, etc. Based on whether or not explicit control messages are required, network tomography could be classified as active tomography~\cite{Rab::MulSouMulDesNT::2004}, \cite{CaceresR::MulInfNetInterLos::1999}, \cite{FraLo::MulInfNetInterDis::2002} and passive tomography~\cite{Y.Var::NTESD::1996}, \cite{JinCao::TimeVarNT::2000}. The former usually actively sends probing packets from the source node and analyzes measurement results at the receivers, while the latter merely utilizes the regularly transmitted data flow for further analysis.



In addition, delay correlation can be further used for topology recovery \cite{BDEriksson::ToPraNTIntTopoDiscov::2010}, \cite{JianNi::EffDynaRouTopoInfEnd2End::2010} that is important to improve network performance. 
